Detecting Deep Neural Network Defects with Data Flow Analysis

Deep neural networks (DNNs) are shown to be promising solutions in many challenging artificial intelligence tasks. However, it is very hard to figure out whether the low precision of a DNN model is an inevitable result, or caused by defects. This paper aims at addressing this challenging problem. We find that the internal data flow footprints of a DNN model can provide insights to locate the root cause effectively. We develop DeepMorph (DNN Tomography) to analyze the root cause, which can guide a DNN developer to improve the model.

==> tex/eval.tex <==
\usepackage{flushend}
\section{experiments}
\label{sec:eval}
We study how \DeepMorph~works in locating defects of DL models via experimental study. 
First, we implement \DeepMorph~over \TensorFlow, a widely-adopted DL software framework. 
Note that \DeepMorph~depends only on the general features of the framework, including obtaining the outputs of hidden layers. 
These features are not specifically available only on \TensorFlow. 
In other words, the \DeepMorph~mechanism can be easily implemented over other DL software frameworks, {\em e.g.}, PaddlePaddle \cite{paddlepaddle}.

\subsection{Experimental Setup}


Our experiments are designed with a focus on answering the following research questions.
\begin{itemize}
    \item {\em RQ1}: How effective \DeepMorph~is in locating model defects in controlled environments.
    \item {\em RQ2}: How \DeepMorph~performs in practical production scenarios.
    \item {\em RQ3}: Whether \DeepMorph~can perform well in different types of DL-based applications
\end{itemize}
 
RQ1 intends to comprehensively study how \DeepMorph~performs in locating DL defects.
Specifically, we evaluate whether \DeepMorph~can figure out three types of model defects. To answer RQ1, we manually inject defects to different types of DL-based computer vision application. \DeepMorph~is then applied to analyze these models with defects.  

RQ2 aims at investigating whether \DeepMorph~is effective to locate model defects in practical production scenario. 
To answer RQ2, \DeepMorph~is applied to DL models trained with larger, more practical production networks designed for computer vision application.

For each experimental setting, we train the corresponding DL model with a set of training data. As we have discussed, \DeepMorph~meanwhile trains its auxiliary \softmax~layers. Then the DL model is applied to a set of testing data, which we use to emulate those encountered in production environments. \DeepMorph~starts to analyze the faulty cases found in the testing data. Specifically, it obtains the possible root cause of each faulty case according to the trend of the rank values, as discussed in Section \ref{sec:method:localization}.
Then for all faulty cases, it produces the ratio of each type of defects.
The defect with the highest ratio value is considered to be the dominant defect of the DL model. To verify whether such a defect causes the bad performance, we also accordingly fix the defect and show the performance improvement of \DeepMorph.




\input{tex/experiment_result.tex}


==> tex/experiment_result.tex <==
\input{tex/tables.tex}

\subsection{Locating model defects in controlled environments}

To answer RQ1, we focus first on computer vision application. 
We conduct experiments on two computer vision datasets, namely, \MNIST~\cite{misc/mnist} and \cifar~\cite{misc/cifar}. 
We train a 5-layer fully-connected network (5-FC) and a LeNet-5 network \cite{nips/CunBDHHHJ89} for the former dataset. We train a LeNet-5 network and an AlexNet network \cite{krizhevsky2012imagenet} for the latter dataset, since it is more complicated. 
To study how \DeepMorph~performs in locating each type of defects, we manually inject the defects to these DL-models and conduct our experimental study, which is elaborated as follows. 

We inject \SD~through manually removing a hidden layer from the original network structures, which aims at degrading the models via a weaker network structure. We train the models  with all correct training data.
To inject \ITD, we randomly choose three target classes and remove 80\% of training data which belong to these three classes, while the testing data remain unchanged. 
In this way, the training data are biased comparing with the testing data.
To inject \UTD, we manually tag a set of faulty labels to some training cases. Specifically, we randomly choose a target class in the training data, and modify 50\% of its labels to another class.

The performance of the DL models with defects, measured by its accuracy in the classification task in testing data, together with the ratio values of defects reported by \DeepMorph~are shown in Table~\ref{exp:fig:ep_1}.

We can see that, for all cases, \DeepMorph~is able to locate the injected defect effectively. According to the ratio values reported by \DeepMorph~, those corresponding to the injected defects are always the largest.
For example, after injecting \UTD~to the \MNIST~data set, the ratio value of \UTD~reaches 0.71 in the 5-FC network, which is the largest comparing with that of \ITD~(0.213) and \SD~(0.077)
This indicates that \DeepMorph~can successfully identified the injected defects.

We then study how \DeepMorph~can help a developer in removing these defects. We assume the developer do not know how the defects are injected. In other words, the DL-models are fixed based only on the outputs of \DeepMorph.

To fix \SD, we add a new layer into the network according to the rank value list obtained by \DeepMorph. Specifically, we choose the hidden layer, where the rank value stop decreasing. We add a layer next to it. 
  
To fixing \ITD, since it is hard in practice to collect new, specifically-selected data for retraining the DL models, we resort to standard data augmentation techniques ({\em e.g.}, random flip and crop) \cite{van2001art}.
We generate a set of new training cases with data augmentation based on the faulty cases that are identified as \UTD~cases.
We then include these generated cases to the biased training data and retrain the model.

To fix \UTD, we perform a manual inspection on the training data and remove falsely-labeled ones. We do not correct the labels since we consider in practice relabeling is labor-intensive, while inspection on the training data can be done via automatic approaches, {\em e.g.}, removing training cases similar to the false cases. 
We therefore also supplement the training data with data augmentation based on the remaining ones.
 
We examine how the DL model performance can be improved, and the data are shown in the ``New Acc.'' column in Table~\ref{exp:fig:ep_1}.  

The results of the experimental study show that \DeepMorph~is capable of detecting the injected defects, and it can help developers to fix the defects effectively. 



\subsection{Evaluation on practical models}

To show the effectiveness of \DeepMorph~in locating model defects in practical production scenarios, we apply \DeepMorph~to DL model trained with the \vggsixteen~\cite{corr/simonyan2014very} network. 
\vggsixteen~is a network widely-adopted in DL-based computer vision application. We train the \vggsixteen~model with \cifar~dataset, without manually injecting any defects.

    
We then use \DeepMorph~directly to the model. The results are shown in Table~\ref{exp:fig:ep2}, with accuracy value equal to 0.681. \DeepMorph~reveals that the dominant defect is \SD, indicating that the structure of \vggsixteen~can be further improved on the \cifar~dataset. 

Hence, we add batch normalization~\cite{ioffe2015batch} and dropout~\cite{srivastava2014dropout} to where the rank value stop decreasing. They aim to increase the generalization capability of the model. We again applied the modified \vggsixteen~network and retrain the model. We can see that the performance is significantly improved to 0.798, which show that fixing the \SD~defect indicated by \DeepMorph~is effective.

This experiment shows that \DeepMorph~can achieve good performance even in locating unknown defects in practical scenarios. With the direction provided by \DeepMorph, the developer can effectively improve DL model performance.

 


==> tex/experiments/exp2_practical.tex <==
\subsection{Evaluation on practical models}
For the sake of fairly evaluating the effectiveness of \DeepMorph\ in practical production scenarios, we consider another two datasets for image classification: \FashionMNIST~\cite{xiao2017/fashion_mnist}, and \SVHN~\cite{netzer2011reading}.
To better simulate the usage scenario of \DeepMorph, we utilize a seven-layer CNN as the network designed by the developer, and VGG-16~\cite{corr/simonyan2014very}, a widely-adopted network in computer vision applications, as the reference network.
The architecture of the seven-layer CNN is shown in Table~\ref{exp:cnn}.
We train the DL classifiers without injecting any defects.


Then we apply \DeepMorph\ directly to these models. 
The performance of the DL models, measured by its accuracy on test data, together with the defect radio reported by \DeepMorph\ are shown in Table~\ref{exp:prac_def}.

We can find that the defect radio of \UTD\ is quite low for every DL model, since the training data are unmodified.
The CNN-7 trained on \FashionMNIST~is reported having \SD, while the remaining all suffering from \ITD.

% why: cnn not good for fashion mnist, no bn for noisy data
% improve
%The results imply that the CNN-7 architecture need to be improved for Fashion-MNIST dataset.
%By contrast, VGG-16 on Fashion-MNIST has the better architecture, and the faulty cases are mainly caused by insufficient training data.
%Comparing to Fashion-MNIST, SVHN is relatively a noisy dataset.

For evaluating how \DeepMorph\ can help a developer in removing these defects, we fix these detected defects accordingly.
For the CNN-7 on \FashionMNIST~dataset has 0.917 accuracy on the test data, but \DeepMorph\ still reports \SD.
So we consider this model encounters overfitting problem and hence add BN layers to this model.
We employ data augmentation techniques to the \ITD\ in other three models.
The accuracy of the improved models are shown in the ``New Acc.'' column in Table~\ref{exp:prac_def}.
We can see that the performance of every model is significantly improved, which show that fixing the defect indicated by \DeepMorph\ is effective.

This experiment shows that \DeepMorph~can achieve good performance even in locating unknown defects in practical scenarios. 
With the direction provided by \DeepMorph, the developer can effectively improve DL model performance.

\input{tex/tables/practical_models.tex}

==> tex/method/method_datafootprint.tex <==

\subsection{Execution footprints of DL models}
\label{sec:method:footprints}

To locate the root cause of bad model performance, we first analyze how an output is produced by a model. 
To facilitate the discussion in this paper, suppose the network has $n+1$ layers, including $n-1$ hidden layers denoted by $l_j$ ($j=1,...n-1$), the input layer $l_0$, and the output layer $l_n$. Let $W_j$ denote the weights of layer $l_jj$, $X_j$ the input to layer $l_j$, $B_j$ the bias, and $g_j(\cdot)$ the activation function. 

As introduced in section~\ref{sec:pre}, the computation of a layer $l_j$ ($j=1,...n$) can be presented as follows.
\begin{equation}
    F_j(X_j) = g_j(W_j \cdot X_j + B_j) 
    \label{eq:layer}
\end{equation}

Note that the output of each layer is fed as the input to its next layer, and the input data are fed from the input layer, processed through every hidden layer, to the output layer.
The entire computational process of a DL model can be treated as the {\em functional} composition of each function $F_j(\cdot)$ of $l_j$.
In other words, since $X_{j+1}=F_j(X_j)$, the output of the model $Y$ given an input $X$ can be written as:

\begin{equation}
    Y = F_n(F_{n-1}(...F_1(X))).
\label{eq:model}
\end{equation}

Similar to the functional programming paradigm where a function's return value depends only on its arguments, for each layer in a DL model, the output is determined by its input.
So every layer in a DL model is {\em idempotent}.
Generally speaking, we can consider each hidden layer $l_j$ conducts some computation $F_j(\cdot)$ to extract specific features from its input $X_j$ via $W_j \cdot X_j + B_j$, and then leveraging the activation function $g_j(\cdot)$ to remove some redundant information while reserving some useful features. For example, the \Relu~activation function will set all negative values to zero and keep all positive values.

Take a classification task ({\em e.g.}, recognizing a handwritten digit) as an example. 
Since a hidden layer $l_j$ takes the output of its previous layer $l_{j-1}$ as input, as the data flow though the network, we can consider that the output data of every hidden layer are made ``distinguishable'' with more distinct features in terms of the classification task. 
It is expected that the features extracted eventually by the last hidden layer can best help the output layer produce a correct result.

%联系program paradigm-
To understand the execution process of a program, traditional approaches generally resort to code coverage metrics ({\em e.g.}, where a line of code is executed). 
But the execution process of a DL model in general cannot be formulated as code coverage, due to its structural specifics~\cite{sosp/PeiCYJ17}.  
In functional programming paradigm, observing whether a function produces the correct result is a common method to locate bugs.
Inspired by the {\em idempotent} character of the layers in DL models, we can consider the intermediate results $X_j$ ($j=2,...n$), given an input, encapsulate all the execution information of a model.
In this regard, intermediate results $X_j$ ($j=2,...n$) are the data flow footprints of how a model processes an input, which can tell why the model produces a correct or incorrect result. This is the basis for \DeepMorph~to perform root cause analysis of bad model performance.

Finally, it is worth noting that the intermediate outputs of every layer typically contain large amount of data, which is too complicated for further analysis. 
\DeepMorph~requires to determine the effective information for the root cause analysis task in the footprints.
Next, we elaborate how \DeepMorph~collects effective information from data flow footprints and accordingly performs root cause analysis of the faulty cases, with a discussion of how \DeepMorph~addresses the above challenges. 

 

==> tex/method/method_defects.tex <==


\subsection{Defects of DL models}
\label{sec:method:defects}

As discussed in Section \ref{sec:pre}, the process of building a DL model typically includes preparing training data and designing the structure of a deep neural network.
It is natural to see that the structure design, including the layers, how layers are connected, and the activation functions, have direct impacts on the model performance. 
In other words, bad performance may result from a bad structure, which we name {\em structure defect}.

%欠拟合+过拟合, underfitting需不需要换个词？
A structure defect may result in {\em underfitting} or {\em overfitting} problem.
Underfitting problem appears when the model is not powerful enough to deal with complicated data.
A simple example could be using a shallow network to deal with complicated machine learning tasks ({\em e.g}, object recognition in real-life images). 
Such a network structure, even trained with correct training data, may not be capable of drawing suitable statistical rules on the data \cite{zhang2016understanding}. 
On the other hand, overfitting refers to the model that fits the training data too well.
The model may learn the details and noises in the training data, which do not apply to new data and negatively impact the model ability to generalize.
Bad performance is then inevitable. 

Although it is straight-forward for an inexperienced developer to instantly blame the network structure if the model encounters poor performance. 
But, the structure defect may not be the sole cause of poor model performance. 
The training data determine the weight parameters of the model via the training process.
The parameters, together with the network structure, determines the correctness of the output given an input. 
Hence, the model performance is determined both by the network structure and the training data. 
Errors in training data also incur bad performance because statistical machine learning, including DL, requires that the training data should bear similar distribution with the data encountered in practical~\cite{books/dl}. 
However, data in the production environment is hard to be obtained and comprehensively analyzed beforehand. 
If the distribution of training data and that of the data encountered in production environment is different, statistical rules learned via the training data cannot be correctly applied in production environment, which will lead to bad performance. 

For example, it is found that a DL-based self-driving car tends to make mistakes in rainy or foggy days~\cite{icse/TianPJR18, kbse/ZhangZZ0K18}. 
The reason is that most of the training data are collected in sunny days. 
The model is biased by such data, resulting in poor performance of the DL-based self-driving car in heavy weather.

Moreover, as we have discussed, training data are in general labeled manually. Human labeling is unreliable in nature. In other words, the training data may contain incorrect labels. Such unreliable training data can mislead the training process and introduce incorrect statistical rules to the model as well.

For example, suppose $a_1$ and $a_2$ are similar cases, both actually belonging to class $A$. 
If $a_1$ is in the training data while being falsely labeled as in class $B$, the model may learn the features of $a_1$ during the training process, and falsely considers them as the the features of class $B$. 
When the model meets $a_2$ in production environment, it may 
conclude that $a_2$ also belongs to class $B$. 
Hence, unreliable training data may also lead to bad performance~\cite{zhang2016understanding}, as we have shown in the motivating example in Section \ref{sec:motivation}.
It is worth noting that locating such defects are not the focus of current DL testing tools, {\em e.g.}, DeepXplore and MODE.

Based on the above discussions, we summarize three representative types of model defects considered in this paper as follows.
\begin{itemize}
\item {\em Structure Defect} (\SD): The improper network structure leads the model to learn inappropriate features from the training data.
\item {\em Insufficient Training Data} (\ITD): The distribution of the training data is different from that of the data in production environment.  
\item {\em Unreliable Training Data} (\UTD): The training set contain falsely labeled cases.
\end{itemize}

For the \SD~case, the developer can improve the structure, {\em e.g.}, with a more powerful network structure, and retrain the model. 
For the \ITD~case, the developer can retrain the model with more data similar to those faulty cases, {\em e.g.}, with data augmentation techniques~\cite{van2001art}, to improve the performance. 
For the \UTD~case, the developer can perform a careful inspection on the training data and correct the errors, and then retrain the model. 
A possible way to reduce human inspection efforts is to focus on the training data that are similar to the faulty cases. 


==> tex/method/method_localization.tex <==
\input{tex/pseudo_code/value_rank.tex}
\subsection{Footprint-based defect localization}
\label{sec:method:localization}
%定义value rank
%由分类正确的case引出value rank的变化重要
%defect分类算法

% introduce value rank and value rank helps
Note that each $S_j$ ($i=1, 2, ..., n$) in the DFS is a vector containing $N$ likelihood values, which implies to what extents the model considers the input case belonging to each target class, according to the extracted features from the corresponding layer.
Given the DFS of an input case belonging to class $c$, we further define the {\em value-rank} of $S_j$, represented by $rv_j$, as the ranking of the likelihood value of the true class $c$ in $S_j$.
For example, $rv_j=2$ means that the input case is deemed as the second most likely belonging to the true class $c$, according to the outputs from layer $l_j$.
Through calculating the value-rank of every $S_j$ in the DFS, \DeepMorph~can obtain the {\em value-rank list} which tracks the variance of the classification results layer by layer when the input case is processed by a DL model.
Algorithm \ref{alg:val_rank} elucidates the procedure for calculating the value-rank list given the DFS of a faulty case in \DeepMorph.

%介绍rank value list变化趋势。。。
We now discuss how DeepMorph uses the value-rank list to localize model defects. 
Let us first suppose the input case is eventually correctly identified as one belonging to $c$ by the DL model. 
The values in the value-rank list can: 1) remain 1 constantly, or 2) be overall ascending and reach 1 in $S_n$. 
Figure~\ref{fig:bug_patterns}(a) shows the examples of such trends, where the $y$-axis represents the value-rank and the $x$-axis represents the layer number.
The first case means the DL model can extract distinct features to successfully classify the case to $c$ even from the lower layers ({\em i.e.}, $l_1$, $l_2$). It indicates the DL model is quite certain that the input belongs to $c$. 
The second case means the DL model can gradually extract distinct features to successfully classify the case to $c$. 
Both cases indicate that the DL model performs as expected: As the data flow thought the network, the output data of every layer are made ``distinguishable'' with more distinct features in terms of the classification task.
 
If the input case is eventually incorrectly identified as one that does not belong to $c$ by the DL model. 
The trend of the value-ranks in the list can exhibit three possible scenarios: 1) The value-ranks in the list are ascending, but do not reach 1 in $S_n$. 2) The value-ranks in the list are descending. 3) The value-ranks in the list remain a relatively constant value other than 1 or oscillating. We also show the examples of these cases in Figure~\ref{fig:bug_patterns}(b)-(d), respectively. 

In the first case, it indicates that the hidden layers have gradually extract useful features from the input case, but they are still not enough even till the output layer. 
As a result, the input case is still misclassified. 
Since the hidden layers have gradually extract more and more distinct features, if the model could be improved ({\em e.g.}, by adding hidden layers), it is quite potential that the value-rank can reach 1 eventually. 
Hence, \DeepMorph~considers that such a trend indicates that the model structure can be improved. 
In other words, \DeepMorph~will report that the DL model has a \SD~defect.

% 总体下降: UTD
In the second case, the overall trend of value-ranks in the list is descending.
The DL model makes mistakes in the very beginning, and even becomes worse till the end.
We consider that the DL model is totally confused about the input case. 
The statistical rules it has learned from the training data cannot apply to the faulty case.
This phenomenon is what we discuss in the motivating example, which shows the model has been trained with similar cases but the cases have a different label other than $c$.
Consequently, \DeepMorph~considers that such a trend indicates a \UTD~defect.

% 其他: ITD
As for the third case, the trend is oscillating, which implies that the statistical rules learned by the model are not obvious in these cases.
This instantly means that such cases are rare in the training data. 
In this regard, \DeepMorph~considers that such a trend indicates an \ITD~defect.

%具体实现，主要介绍threshold
Algorithm \ref{alg:localize} demonstrates the implementation of defect localization in \DeepMorph.
\DeepMorph\ summarizes the ascending and descending trend of two consecutive value-ranks in the list, and thus determine the overall trend of value-ranks.
For example, if the number of ascending value-rank pairs is less than the manually-set threshold, then \DeepMorph\ determines the overall trend of value-ranks is descending and considers the faulty case is caused by \UTD.
Since DL models may consist of tens to hundreds number of layers, the thresholds are set according to the total number of layers in the target model.
Specifically, the thresholds for ascending and descending both by default are set to $\lceil0.2n\rceil$ in \DeepMorph, where $n$ is the total number of layers in the target model.

To sum up, \DeepMorph~analyzes the trends of the value-ranks to perform root cause analysis of bad performance.
We evaluate how \DeepMorph~works in our experimental study next.


% 改图。。。！！！ 
\begin{figure}[t]
\centering
\subfigure[Correct cases]{
\includegraphics[width=0.46\linewidth]{fig/methodology/correct.png}
\label{fig:bug_pattern:1}
}
\subfigure[Faulty case 1]{
\includegraphics[width=0.46\linewidth]{fig/methodology/SD.png}
\label{fig:bug_pattern:2}
}
\subfigure[Faulty case 2]{
\includegraphics[width=0.46\linewidth]{fig/methodology/UTD.png}
\label{fig:bug_pattern:3}
}
\subfigure[Faulty case 3]{
\includegraphics[width=0.46\linewidth]{fig/methodology/ITD.png}
\label{fig:bug_pattern:4}
}
\caption{Examples of the trend of value-ranks collected from a 5-layer model trained on MNIST}
\label{fig:bug_patterns}
\end{figure}

\input{tex/pseudo_code/defect_rule.tex}

==> tex/method/method_modeling.tex <==
\subsection{Modeling execution footprints}
\label{sec:method:def_dis}
 
A straight-forward approach to analyze a faulty case is to compare the execution process of how the model processes the faulty cases with that of how it processes correct cases. 
As we have discussed, the intermediate results $X_j$ (j$ = 2, ...n$) of each hidden layer reflect the execution process of a model.
Hence, we propose to make use of the intermediate outputs of hidden layers for defect localization.
Specifically, \DeepMorph~compares the execution processes of how the model processes a faulty case and the training cases via extracting footprint specifics from such data flow footprints.

Let us suppose there are $M$ training cases for a classification task, each labeled as one of the $N$ classes. 
Class $k$ ($k = 1,..,N$) contains training case set $M_k$. 
The data flow footprints of the training cases in $M_k$ form a set $t_k$, and those of the faulty cases are denoted by $f_k$.

To compare the execution processes for the faulty cases and those of the training cases, one may instantly suggest to compare the distributions of $t_k$ with $f_k$. 
Specifically, we can compare the distributions of intermediate outputs of $M_k$ from each hidden layer with those of faulty cases to investigate how the cases are eventually misclassified. 
As discussed in Section~\ref{sec:method:footprints}, 
according to the functional nature of deep neural networks, it is expected that each hidden layer extracts more and more subtle features that can help the output layer correctly perform the machine learning task.
The output data of each hidden layer, from $l_1$ to $l_{n-1}$, should tend to be more distinguishable in terms of the classification task. 
Therefore, comparing the feature of the faulty case extracted in each layer with that of each $M_k$ in the training data can help us understand whether the features of the faulty case are correctly extracted. 
For example, we can see whether such features are getting less distinguishable or whether it persistently misleads the model to misclassification.

A widely-adopted way to compare a data item ({\em i.e.}, $X_j$ for the faulty case) to the distribution of a set of data items ({\em i.e.}, all the $X_j$ data for the training cases) is to calculate their Mahalanobis distance~\cite{de2000mahalanobis}.  
However, calculating Mahalanobis distance is computation-intensive, especially when there are tremendous training cases and the data volume of the intermediate results $X_j$ (j$ = 2, ...n$) are huge.
Moreover, such a distance can best model how close a point is to a distribution based on the assumption that the distribution is Gaussian~\cite{de2000mahalanobis}, which may not hold for the intermediate results. 

To deal with the huge volume of the intermediate results, we propose to perform additional feature extraction of the intermediate results $X_j$.   
Actually, the underlying idea of the Mahalanobis-distance proposal is that we should track whether the features of the faulty cases are correctly extracted in the hidden layers.  
Inspired by the functionality of the \softmax~activation function typically used in the output layer, which produces the likelihood of that the input belongs to each class, {\em q.v.} Equation (\ref{eq:softmax}), 
we use a \softmax-based approach to extract the footprint specifics of faulty cases.

\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{fig/aux_layers.png}
\caption{Overview of the softmax-instrumented model}
\label{fig:hidden_extractor}
\end{figure}

Specifically, \DeepMorph~resorts to an auxiliary \softmax\ layer connected to each hidden layer in the target model, and builds the \softmax-instrumented model so as to extract the footprint specifics. 
Figure~\ref{fig:hidden_extractor} shows how such auxiliary \softmax\ layers are connected to the original deep neural networks via a simple example. 
For an $N$-class classification task, an auxiliary \softmax\ layer contains $N$ neurons. 
Each hidden layer is fully-connected to one particular auxiliary \softmax\ layer. 
In other words, each neuron in the auxiliary \softmax\ layer connects to all neurons in the hidden layer.

We can consider that the \softmax-instrumented model is a new neural network that outputs the likelihood, in the view of each hidden layer, that the input case belongs to each target class. 
We adopt such likelihood data to model whether the features of an input case are correctly extracted by the hidden layers.
Just like other DL models, we first need to train the parameters of the \softmax-instrumented model.

Note that our focus is to compare intermediate results of training data $t_k$ ($k=1,2,...,N$) with those of the faulty case $f_k$ in each hidden layer of the original model, we only need to train the parameters of auxiliary \softmax~layers with $t_k$.

Specifically, \DeepMorph\ freezes all parameters in the original model during the training progress.
Then \DeepMorph\ use the same training data to train the \softmax-instrumented model.
When the training data is processed by each hidden layer, the intermediate outputs not only flow to the next layer, but also to the corresponding auxiliary \softmax\ layer.
Since the parameters of the original model are frozen, the intermediate results $X_{j+1}$ can be calculated correctly and then used to train the corresponding auxiliary \softmax\ layer with the label of training data.
In this way, \DeepMorph\ train the \softmax-instrumented model that can be used to extract the footprint specifics of the faulty cases.

Specifically, given an input, let $S_j$ denote the output of the auxiliary \softmax\ layer corresponding to hidden layer $l_j$.  
$S_j$ is a vector of size $N$, where each element represents the likelihood that the input case belongs to each target class, according to the intermediate results $X_j$.

Note that the output layer uses the \softmax\ activation function as well, so the output of the original DL model $S_n$ is a vector similar to $S_j$ ($j=1, 2, ..., n-1$).
We consider the outputs of all the the auxiliary \softmax\ layers, together with the final output $S_n$, can describe the data flow footprint specifics of the input. In other words, it describes how the DL model processes the input. We let \DFS\ denote such footprint specifics, presented as follows. 
\begin{equation}
    DFS = [S_1, S_2, ..., S_{n-1}, S_n]
\label{eq:dft}
\end{equation}
In Section \ref{sec:method:localization}, we will elaborate how \DFS\ can help locate model defects.

%Finally, note that \DeepMorph~requires the intermediate results $X_j$ to obtain \DFS. 
%This is in general feasible in modern DL software framework.
%Take \TensorFlow, a widely-used DL framework, as an example. \TensorFlow~employs a directed graph to describe a dataflow of computation~\cite{osdi/AbadiBCCDDDGIIK16}.
%Each node in the graph represents an operation with a unique name, {\em i.e.}, 'layer:operation:0'.
%Since each hidden layer $l_j$ in the DL model has an activation function and its output is $X_{j+1}$, \DeepMorph~only need to obtain all the operation names associated with activation function from the built-in \emph{Graph} structure.
%The outputs of the operation ({\em i.e.}, $X_{j+1}$) can then be retrieved by the \texttt{get\_tensor\_by\_name} method in \TensorFlow.



==> tex/motivation.tex <==

\section{Motivation}
\label{sec:motivation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/motivation/mnist_code.png}
    \caption{Source code of a simple deep neural network model}
    \label{mov:fig:dnn_code}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{fig/motivation/err_imgs.png}
    \caption{Original faulty cases with digit '4' but recognized as '9' included}
    \label{mov:fig:err_imgs}
\end{figure}

\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{fig/motivation/4vs9.png}
\caption{T-SNE results of right and faulty cases with label '4' and '9'}
\label{mov:fig:im_data}
\end{figure*}

DL models generally cannot achieve 100\% accuracy due to its basis: it draws rules statistically according to the training data. 
When deployed in a production environment, it may encounter inputs that do not follow the statistical rules, and consequently produces faulty results~\cite{books/dl}. 

When a DL developer builds a model for a specific task, it is quite hard for her to understand whether there is room to improve its performance. 
For example, suppose she builds a deep neural network model to recognize flowers, and
the model achieves 80\% accuracy in the production environment ({\em i.e.}, 20\% of the inputs are misclassified). It is in fact a very challenging problem for her to tell whether and how this accuracy can be improved. 
She may make mistakes in building the model, which bring defects to the model. Such defects can then possibly be fixed to improve the accuracy.

Such a problem is more severe as deep learning surges into popularity recently. 
More and more developers, who may not be experienced machine learning practitioners, have included deep learning techniques into their applications.

We further illustrate this problem with a simple motivating example. 
Let us suppose a developer builds a simple DNN model to recognize digits.
The developer trains the network with \MNIST~\cite{misc/mnist}, a widely-adopted handwritten digits dataset. 
With modern deep learning software framework, {\em e.g.}, \TensorFlow, it is quite convenient for her to build her own models.
Suppose she builds a five-layer (excluding the trivial input layer by convention) network with \TensorFlow. 
To facilitate our discussions, we name these layers $l_1$, ..., $l_5$ respectively, where $l_1$ connects to the input layer and $l_5$ is the output layer.

We show her codes in figure~\ref{mov:fig:dnn_code}, which contain three parts: loading the \MNIST~dataset, defining the network structure, and training the model with the data.
We can see that the implementation is quite easy to follow. 
But simple as it shows, the codes may still produce a model with low accuracy in recognizing digits. 
For example, the model may be trained with improper training cases, where these cases bear different statistical characteristics with those that can be met in practice. 
As a result, the network is misled by the training data, and generates a model with wrong statistical rules.
Poor accuracy is then inevitable in practice.

For illustration purpose, consider in the training data some images that actually contain digit '4' are wrongly labeled as those including '9'.
Note that in typical machine learning application, training data are manually labeled usually.
Errors in training data introduced due to human factors are not rare cases \cite{zhang2016understanding}. 

After the developer trains the model with the data that contains errors, the model is applied to recognize handwritten digits. 
Figure \ref{mov:fig:err_imgs} shows a set of errors the model produces, where the images containing digit '4' are misclassified as those containing the digit '9'. 
We can see that with these faulty cases only, it is still hard for the developer to know whether she has mistakenly introduced defects to the model, and if so, how to locate the root cause. 
Current tools, {\em e.g.}, DeepXplore and DeepTest, generally focus on generating effective testing cases. 
They cannot help the developer to pinpoint the defects as well.

As we have discussed in Section \ref{sec:pre}, an output is produced after data flow from the input layer, processed by every hidden layer, to the output layer. 
Motivated by such a nature of neural networks, we consider that the internal data flow footprints ({\em i.e.}, the output of each layer $l_i$), may shed light to locating the root cause of the faulty cases. 

To this end, we compare how similar a {\em faulty} case ({\em i.e.}, digit '4' wrongly identified as '9') to those {\em correctly} identified as digit '4' and those {\em correctly} identified as digit '9'. 
For the output in every layer from three kinds of cases, we use the t-distributed stochastic neighbor embedding (t-SNE) algorithm~\cite{maaten2008visualizing}, which is commonly used for data exploration and visualization, to visualize these high-dimensional data.

%宏观描述一下图
The visualization results is shown in figure~\ref{mov:fig:im_data}, where every shape represents the intermediate output of one test case from the corresponding layer, the distance between two shapes reflects the similarity of the outputs. 
We can find that the intermediate outputs of correct test cases are promiscuous in layer $l_1$, separable in layer $l_3$, and totally separated in layer $l_5$.
We pay attention to the output of faulty cases that wrongly identified as '9' instead of '4', especially from layer $l_3$ to $l_5$ since the outputs of latter layers are more distinguishable than previous ones.

%分段介绍error cases
%poisoned data
It is worth noting that the output of faulty case 1 in each layer $l_i$ is closer to the outputs of correct '9' cases, comparing with those of the correct '4' cases. 
In other words, the model has wrongly consider a '4' in the faulty case as a '9' from the very beginning ({\em i.e.}, $l_1$), throughout every hidden layers, and recognize it as a '9' eventually in the output layer. 
Although the original case is like a '4' to a human being (see figure~\ref{mov:fig:err_imgs}), the model have persistently considered the faulty case is more similar to a '9'.
One can consider that such a progress of yielding the wrong result '9' indicates the model is quite certain that the faulty case is a '9', although it is a '4' to a human being. 
The developer may then conclude the model has been trained with such similar cases (where '4' labeled as '9'), so that the model considers the faulty case is a '9' throughout all the hidden layers. 

%structure defect
On the other hand, the outputs of faulty case 2 are more similar to correct '9' cases in layer $l_1$ to $l_3$, and become closer to correct '4' cases in layer $l_4$ and $l_5$. 
Indeed, the model extracted informative features from these faulty cases, while the extracted features may be not effective enough to produce the correct results.
The developer may consider to improve the representation power of the model by changing the model structure.

To this end, she can then be directed to inspect the training cases, remove those wrongly-labeled data, and train a new model with new structure using the polished training data. 
 
In conclusion, when a DL model suffers bad performance, it is hard for its developer, especially an inexperienced one, to figure out whether the results are reasonable or caused by her mistake.
The above motivating example demonstrates that it is promising to pinpoint the root cause with the internal data flow footprints.
This work aims at designing and implementing a tool that can automatically analyze the defects in DL models via considering the internal data flow footprints, and direct developers to effectively enhance the model. 


==> tex/preliminaries.tex <==
 \section{preliminaries}
\label{sec:pre}

\begin{figure}[t!]
\centering
\subfigure[Neural network structure]{
\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/simple_nn.png}
\label{pre:fig:model:1}
\end{minipage}
}
\subfigure[Neuron computation process]{
\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/neuron.png}
\label{pre:fig:model:2}
\end{minipage}
}
\caption{A simple neural network model}
\label{pre:fig:model}
\end{figure}

Deep neural networks (DNNs) are designed to automatically draw statistical rules from training data~\cite{books/dl}.
In this section, we introduce preliminary knowledge on DNNs with a focus on their typical structures.

A DNN usually consists of a number of neurons with a layered, connected structure, where a \textit{neuron} is the basic computational unit.
Figure~\ref{pre:fig:model:1} shows the structure of a simple neural network.
Each connection between two neurons, shown as a line in the figure, represents a data flow link in the network, which is decorated with a \textit{weight} parameter.

% neuron introduction
A neuron can then calculate the weighted sum of all its inputs, add a bias, and finally evaluate its output with an \textit{activation function}, as shown in Figure~\ref{pre:fig:model:2}.
Specifically, the output is $g(\sum_{\forall i \in input} (weight_i \cdot input_i) + bias)$.
The activation function $g(\cdot)$ is typically a non-linear function, which introduces non-linear property to a network. A network can thus perform non-linear calculation.
In other words, it is capable of fitting a complicated function, which is critical to deal with complicated data such as images, audio, and videos.
The most widely-used activation function is the \Relu~(Rectified Linear Unit) function~\cite{icml/NairH10}.

% layer introduction
A \textit{layer} in a network can be considered as a set of neurons that locate at the same level in the network structure, where neurons in the same layer will not connect to each other.
A network includes an \textit{input layer}, one or many \textit{hidden layers}, and an \textit{output layer}. The input layer directly connects to the input data ({\em i.e.}, a vector), where each neuron connects to one dimension of the data.
The hidden layers are typically designed to extract multiple levels of representations and abstraction from the input data.
Data flow from the input layer, calculated by neurons in between, to the output layer so as to yield a result.
For example, an image can go through a network and output the object it contains ({\em e.g.}, a flower, a bird, or  an aircraft).

To deal with multi-class classification problems ({\em i.e.}, determining which class in $n$ classes the input belongs to), the output layer commonly uses the \softmax~activation function.
It is shown below, where $(x_1, x_2, ..., x_n)$ is a vector of the inputs to the \softmax~function, and $i$ is the index of each target class.
\begin{equation}
    d_i = \sigma(x_i)=\frac{e^{x_i}}{\sum_{j=1}^{n}e^{x_j}}
    \label{eq:softmax}
\end{equation}
The output of this function is a vector of size $n$. The value of each element $d_i$  ($i$ = 1, 2, ..., $n$) of the vector is in interval [0, 1].
Moreover, $\sum_{i=1}^{n} d_i = 1$. In this way, $d_i$ represents how likely the input belongs to class $i$.

Essentially, a DL practitioner will typically design the {\em structure} of the proposed DNN, where she will design the layers, how layers are connected, and the activation functions.
The network structure is specifically tailored for a problem domain. For example, the VGG-16 structure is designed for object image recognition~\cite{corr/simonyan2014very}.
The training process of a neural network is to find the weights so that the output can best produce expected results, typically with backpropagation~\cite{nips/CunBDHHHJ89}.

Finally, it is straight-forward to know that a network, together with the weight parameters between neurons, determines how it processes the input to generate output.
We call a network (including the weight parameters between neurons and the network structure) a {\em DL model}, or in short, a model. The performance of a model, {\em i.e.}, whether it can produce correct output given an input, is largely determined by the weight parameters and the network structure. Since the parameters are obtained during the training process with the training data, the performance is determined by the network structure and the training data.

 
 






==> tex/pseudo_code/defect_rule.tex <==
\begin{algorithm}[ht]
    \small
	\caption{Defects Localization}  
	\label{alg:localize}
	\begin{algorithmic}[1]
		\Require the Value-Rank of a incorrect case $\mathbf{vr}$, the layer number of model $L$
		\Ensure a vote of the DL model's primary defect $defect$, which is $\in \{\mathbf{ITD}, \mathbf{UTD}, \mathbf{SD}\}$
		\State $//vr_{i}\ is\ the\ Value$-$Rank\ of\ i$-$layer\ in\ \mathbf{vr}$
		\State $lt \gets 0$, $gt \gets 0$
		\For{$i := 1 \to L$}
			\If{$i == 1$}
				\State $Rank_{last} := vr_{i}$
			\Else
				\State $Rank_{cur} := vr_{i}$
				\If{$Rank_{cur} < Rank_{last}$}
					\State $lt := lt + 1$
				\ElsIf{$Rank_{cur} > Rank_{last}$}
					\State $gt := gt + 1$
				\EndIf
				\State $Rank_{last} := Rank_{cur}$
			\EndIf
		\EndFor
		\If{$lt < threshold_{sd}$}
			\State $defect := \mathbf{SD}$
		\ElsIf{$gt < threshold_{utd}$}
			\State $defect := \mathbf{UTD}$
		\Else
			\State $defect := \mathbf{ITD}$
		\EndIf
	\end{algorithmic}  
\end{algorithm}  	

==> tex/pseudo_code/value_rank.tex <==
\begin{algorithm}[h] 
    \small
	\caption{Value-Rank Extraction} 
	\label{alg:val_rank}
	\begin{algorithmic}[1]
		\Require true label $c$, dataflow footprint specifics $\mathbf{DFS}$, the number of DL model layers $n$
		\Ensure the value-rank list of one input $\mathbf{vrl}$
		\State $\mathbf{vrl} := \varnothing$ 
		\For{$i := 1 \to n$} \\
			//function $\mathbf{argsort}$ sorts index by value in descending order
			\State $S_{argsort} := \mathbf{argsort}(S_{i})$
			\State $vr_{i} \gets \mathbf{arg}\{S_{argsort} = c\}$
			\State $\mathbf{vrl} := \mathbf{vrl} + vr_{i}$
		\EndFor
	\end{algorithmic}  
\end{algorithm}

==> tex/tables/practical_models.tex <==
\begin{table}[htbp]
    \centering
    \caption{Results on practical DL models}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Acc.}} & \multicolumn{3}{c|}{\textbf{Defect Radio Reported}} & \multirow{2}{*}{\textbf{New Acc.}} \\
        ~ & ~ & ~ & \textbf{ITD} & \textbf{UTD} & \textbf{SD} & ~ \\
        \midrule
        \multirow{2}{*}{\textbf{Fashion-MNIST}} & \textbf{CNN-7} & 0.917 & 0.28 & 0.106 & {\color{red}\textbf{0.614}} & 0.928 \\
        ~ & \textbf{VGG-16} & 0.895 & {\color{red}\textbf{0.768}} & 0.01 & 0.222 & 0.9315 \\
        \midrule
        \multirow{2}{*}{\textbf{SVHN}} & \textbf{CNN-7} & 0.894 & {\color{red}\textbf{0.469}} & 0.278 & 0.253 & 0.922 \\
        ~ & \textbf{VGG-16} & 0.927 & {\color{red}\textbf{0.944}} & 0.01 & 0.046 & 0.956 \\
        \bottomrule
    \end{tabular}
    }
    \label{exp:prac_def}
\end{table}
